Towards Robust and Efficient Communications for Urban Air Mobility

For the realization of the future urban air mobility, reliable information exchange based on robust and efficient communication between all airspace participants will be one of the key factors to ensure safe operations. Especially in dense urban scenarios, the direct and fast information exchange between drones based on Drone-to-Drone communications is a promising technology for enabling reliable collision avoidance systems. However, to mitigate collisions and to increase overall reliability, unmanned aircraft still lack a redundant, higher-level safety net to coordinate and monitor traffic, as is common in today's civil aviation. In addition, direct and fast information exchange based on ad hoc communication is needed to cope with the very short reaction times required to avoid collisions and to cope with the the high traffic densities. Therefore, we are developing a \ac{d2d} communication and surveillance system, called DroneCAST, which is specifically tailored to the requirements of a future urban airspace and will be part of a multi-link approach. In this work we discuss challenges and expected safety-critical applications that will have to rely on communications for \ac{uam} and present our communication concept and necessary steps towards DroneCAST. As a first step towards an implementation, we equipped two drones with hardware prototypes of the experimental communication system and performed several flights around the model city to evaluate the performance of the hardware and to demonstrate different applications that will rely on robust and efficient communications.

==> Discussion.tex <==
\section{Discussion with Respect to Project HorizonUAM}
\textcolor{red}{Welchen Beitrag leisten die Lösungen, um die Kosten zu minimieren, den Nutzen zu maximieren und die gesellschaftliche Akzeptanz zu steigern?
\begin{itemize}
	\item Kollisionswahrscheinlichkeit wird verringert
	\item gesellschaftliche Akzeptanz wird erhöht
	\item Erkenntnisse aus Kanalmessungen und Kanalmodell helfen bei Design und Evaluierung von Kommunikationssystemen im urbanen Umfeld
	\item DroneCAST ist eine technische Lösung
\end{itemize}
\begin{itemize}
	\item Ausgangssituation und technologische Entwicklung, wo sind Lücken?
	\item UAM muss sicher sein!
\end{itemize}
}

\paragraph{Stand der Technik}

\paragraph{Lösungsansatz mit Bezug zu Projektergebnissen}

\paragraph{wichtigste Ergebnisse und Bewertung der Beiträge zu UAM erläutern}


